CenterGrasp: Object-Aware Implicit Representation Learning for Simultaneous Shape Reconstruction and 6-DoF Grasp Estimation

Reliable object grasping is a crucial capability for autonomous robots. However, many existing grasping approaches focus on general clutter removal without explicitly modeling objects and thus only relying on the visible local geometry. We introduce CenterGrasp, a novel framework that combines object awareness and holistic grasping. CenterGrasp learns a general object prior by encoding shapes and valid grasps in a continuous latent space. It consists of an RGB-D image encoder that leverages recent advances to detect objects and infer their pose and latent code, and a decoder to predict shape and grasps for each object in the scene. We perform extensive experiments on simulated as well as real-world cluttered scenes and demonstrate strong scene reconstruction and 6-DoF grasp-pose estimation performance. Compared to the state of the art, CenterGrasp achieves an improvement of 38.5 mm in shape reconstruction and 33 percentage points on average in grasp success. We make the code and trained models publicly available at http://centergrasp.cs.uni-freiburg.de.

==> tables/grasp_results.tex <==
\begin{table}[t]
\centering
\caption{Evaluation of 6-Dof grasp pose predictions in simulation. Results are averaged over 3 random seeds. \textit{SR = Success Rate ($\uparrow$), DR = Declutter Rate ($\uparrow$).}}
\label{tab:grasp-results}
\begin{tabularx}{0.85\columnwidth}{l c c c c c}
\cmidrule{1-6}
Method & \multicolumn{2}{c}{Packed} && \multicolumn{2}{c}{Pile} \\ 
\cmidrule{1-6}
& SR & DR  && SR & DR \\
\cmidrule{2-3} \cmidrule{5-6}
GIGA~\cite{jiang2021synergies} 
& 0.52 & 0.58 && 0.43 & 0.17 \\
CenterGrasp w/o ICP 
& 0.23 & 0.16 && 0.17 & 0.13  \\
CenterGrasp
& \textbf{0.83} & \textbf{0.86} && \textbf{0.86} & \textbf{0.71}  \\ 
\cmidrule{1-6}
\end{tabularx}
\end{table}

==> tables/reconstruction_pose_results.tex <==
% \begin{minipage}[c]{0.48\textwidth}
%     \centering
%         \begin{tabular}{l|ccc}
%             \toprule
%             Method & CD (Bi) & CD (Uni) & \rebuttal{IoU} \\ 
%             \midrule
%             GIGA~\citep{jiang2021synergies}  & 77.0 & 41.0 & \rebuttal{0.16} \\
%             \ourName{} & \textbf{34.7} & \textbf{19.4} & \textbf{\rebuttal{0.84}} \\
%             \bottomrule
%         \end{tabular}
%     % \medskip
%     \captionof{table}{Reconstruction Results. We compute the bi- and uni-directional L2-Chamfer distance (CD) ($\downarrow$) multiplied by 1000, \rebuttal{and the IoU ($\uparrow$) between reconstructiona and object's point cloud.}}
%     \label{tab:reconstruction-results}
% \end{minipage}
% \hfill
% \begin{minipage}[c]{0.48\textwidth}
%     \centering
%         \begin{tabular}{l|ccc}
%             \toprule
%             Method & $5\degree$5cm & $10\degree$10cm & $15\degree$15cm \\ 
%             \midrule
%             Loss by \cite{irshad_centersnap_2022}  & 30.2 & 60.2 & 74.3 \\
%             \ourName{} & \textbf{54.7} & \textbf{76.4} & \textbf{84.1} \\
%             \bottomrule
%         \end{tabular}
%     % \medskip
%     \captionof{table}{Pose Estimation Results. Following \cite{wang_normalized_2019} we compute the average precision ($\uparrow$) for poses thresholded by rotation and translation error jointly.}
%     \label{tab:pose-results}
% \end{minipage}

\begin{table}
\centering
\caption{Reconstruction Results. We compute the bi- and uni-directional L2-Chamfer distance (CD) ($\downarrow$) multiplied by 1000, and the IoU ($\uparrow$) between reconstruction and object's point cloud. Results are averaged over 3 random seeds.}
\label{tab:reconstruction-results}
\begin{tabular}{l|ccc}
    \toprule
    Method & CD (Bi) & CD (Uni) & IoU \\ 
    \midrule
    GIGA~\cite{jiang2021synergies}  & 35.6 & 21.7 & 0.18 \\
    \ourName{} & \textbf{23.2} & \textbf{10.6} & \textbf{0.33} \\
    \bottomrule
\end{tabular}
% \medskip
\end{table}


==> tables/timing_results.tex <==
% \begin{table}[htbp]
%     \centering
%         \begin{tabular}{l|ccc}
%             \toprule
%             Task & 1 Object & 3 Objects & 5 Objects \\ 
%             % \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
%             \midrule
%             Image Encoding \\
%             SGDF Reconstruction \\
%             ICP \\
%             Grasp Filtering \\
%             \eugenio{something?} \\
%             \midrule
%             Total [s] & 0.615 & 0 \\
%             \bottomrule
%         \end{tabular}
%     \medskip
%     \caption{Breakdown of \ourName's Inference Time Rates. \eugenio{add more explanation here.}}
%     \label{tab:timing-results}
% \end{table}

\begin{table}[htbp]
    \centering
        \begin{tabular}{l|ccc}
            \toprule
            Task & w/o ICP & with ICP \\ 
            \midrule
            Image Encoding & 0.101 & 0.101 \\
            SGDF Reconstruction & 0.816 & 0.816 \\
            ICP & N/A & 0.041\\
            Grasp Filtering & 2.398 & 0.911\\
            \midrule
            Total & 3.315 & 1.869 \\
            \bottomrule
        \end{tabular}
    \medskip
    \caption{Breakdown of \ourName's Inference Time Rates in [s]. We report the inference time for 3 objects visible in the scene and give a breakdown. \eugenio{Numbers not final (taken from different (slower) pc)} \eugenio{add more explanation here.}}
    \label{tab:timing-results}
\end{table}
